AUGUR, A flexible and efficient optimization algorithm for identification of optimal adsorption sites

In this paper, we propose a novel flexible optimization pipeline for determining the optimal adsorption sites, named AUGUR (Aware of Uncertainty Graph Unit Regression). Our model combines graph neural networks and Gaussian processes to create a flexible, efficient, symmetry-aware, translation, and rotation-invariant predictor with inbuilt uncertainty quantification. This predictor is then used as a surrogate for a data-efficient Bayesian Optimization scheme to determine the optimal adsorption positions. This pipeline determines the optimal position of large and complicated clusters with far fewer iterations than current state-of-the-art approaches. Further, it does not rely on hand-crafted features and can be seamlessly employed on any molecule without any alterations. Additionally, the pooling properties of graphs allow for the processing of molecules of different sizes by the same model. This allows the energy prediction of computationally demanding systems by a model trained on comparatively smaller and less expensive ones

==> chapters/Intro_usecase_systems.tex <==
To demonstrate the efficacy of our method, we use the following two different systems we encountered in our previous research:
First, we considered chini clusters[do we need a Reference here?], which are a unique class of organometallic compounds known for their interestingly unusual bonding and electronic properties. Their interaction with Zn(2+) ions served as a good starting model in our previous exhaustive combined experimental and theoretical study that focussed on understanding the chemistry of atom-precise Pt Np encapsulation inside a ZIF-8, which helps in inhibiting the agglomeration of small Pt-Np-precursors due to their high Surface energy [reference]. ZIF-8 is a Molecular Organic framework that consists of Zn(2+) ion as the node; its interaction with the Pt Np precursor (Chini cluster) plays a vital role in the self-assembly of the MOF precursors around the Nps. A method to screen the starting positions of Zn(2+)-Chini cluster interactions will surely be of help to expediate the process of finding the most important active sites on the cluster.


% Chini Clusters serve as an interesting class of materials to be used as precursors of atom-precise nanoparticles. There precursors interact with the host system to confine the growth of Nps and decrease agglomerative tendencies due to high surface energy of the small NPs. We chose this system as we already have extensive experimental and theoretical study of their interactions with the ZIF8 node, Zn2+. This helped us in confirming the reliability of our ML model. 

% \end{itemize}
% \subsection{Second subsection}
% \begin{itemize}
%     \subsection{Study 1: Zn adsorption on Pt-Chini clusters} 
%     \item {Basic info about Pt-Chini Clusters, why do we need to study Zn interaction with these clusters and why specifically chini clusters for the study } 
    
%     \subsection{Study 2: Carbon Monoxide adsorption on ZnO clusters}
%     \item {About ZnO clusters, why CO adsorption on ZnO clusters, previous studies and shortcomings in studying ZnO clusters, and why esp. ZnO clusters for this study}
% \end{itemize}


Second, we selected ZnO clusters that are well-known experimentally to be used in semiconductor companies for chips, sensors, and electrodes due to their observed high catalytic activity and stability.[Reference?] In our study, the focus lies on the gas adsorption capability of the \ch{(ZnO)78} cluster, as it is one of the "magic clusters", but it has not yet been studied in depth. \ch{(ZnO)78} can form a double-caged structure \cite{Vines.2017}, where a smaller \ch{(ZnO)18} cage lies within a larger \ch{(ZnO)60} cage. This structure is shown in \Cref{figures/zno/fig:ZnO78}. Other geometries, e.g. a sodalite structure \cite{Wang.2010} or a nested structure \cite{Dmytruk.2017}, have also been proposed. The adsorption energy can be calculated by comparing the energy of the combined system to the sum of the energies of the isolated systems:
% \includegraphics[width=\linewidth]{figures/pt/Pt6_cropped.png}

\begin{equation}
    \label{eq:adsorption-energy}
    E_{\mathrm{ads}} = E_{\mathrm{cluster + \ch{CO}}} - (E_{\mathrm{cluster}} + E_{\mathrm{\ch{CO}}}),
\end{equation}
where $E_{\mathrm{ads}}$ is the adsorption energy, $E_{\mathrm{cluster +\ch{CO}}}$ is the energy of the combined system after the adsorption of \ch{CO} to the cluster, and $E_{\mathrm{cluster}}$ and $E_{\mathrm{\ch{CO}}}$ are the energies of the isolated systems.

The energies of the different systems are calculated based on Density Functional Theory (DFT). However, due to the large size of the cluster, the conventional approach of exhaustive DFT investigation, covering the entire surface of the cluster, is computationally infeasible. Therefore, we propose to speed up the process by using Graph powered Bayesian optimization incorporated into AUGUR.

==> chapters/ML_parameters.tex <==
% The graph neural networks have been trained using NN convolutions inspired by \cite{NNCONV_1,NNCONV_2} and normal batch normalization layers. The number of layers scaled with the number of atoms in the system, with the Pt clusters requiring 2 convolution layers and the (ZnO)$_{78}$ 3. The network has been implemented in \cite{pytorch_geometric}.  The pooling layers consisted of a mean and a max pooling.
% The Gaussian Processes use a Linear mean and a spectral mixture kernel inspired by \cite{spectral_mixture} and implemented in gpytorch \cite{gpytorch}. The code for the full model, containing all the parameters and algorithms used will be made publicly available by providing a git repository in this section upon acceptance of the manuscript.

==> chapters/simulation_methodologyZNO.tex <==
% We utilized the DFT Framework implemented in two software packages (ORCA and CP2K) [42] [43] to generate  the dataset of the two use case systems shown in \Cref{fig:pt_clusters} and \Cref{fig:zn_cluster} 
% % BO optimization scheme. The DFT optimizations aimed to create a dataset that includes the physically viable
% % cluster-molecule/ion interacting structures and their corresponding energies. These specific use case systems
% % were selected to cover different classes of materials—from metal-carbonyl coordination compounds to inorganic
% % semiconductor systems—due to numerous literature studies to compare with and their relative simplicity. This
% % selection was intended to facilitate testing the model’s generalizability 

% The DFT simulations generated a dataset of the physically viable cluster-adsorbate interacting structures and their corresponding energies. 
% These structures are extracted from the relaxation trajectory paths based on ['IOANNIS; how did you select specific iterations?--- Mention selection of dissimilar coordinates- reason- covariance matrix giving 0 trace?']. 
% These specific use case systems were selected to cover different classes of materials—from metal-carbonyl coordination compounds to inorganic semiconductor systems—due to numerous literature studies to compare with and their relative simplicity. This selection was intended to facilitate testing the model's generalizability.


% \subsection{ System 1: Chini Clusters}
   
    
% The geometry optimizations of the chini clusters (Pt$_{3}$, Pt$_{6}$, Pt$_{9}$) were done using the DFT method implemented in the quantum chemistry software ORCA 5.0.4 \cite{Orca-Neese2012}. The structures of the bare clusters and their initial interactions with the Zn$^{(2+)}$-ZIF8 node, placed at chemically distinct sites, were optimized in a methanol solvent, modeled by the CPCM implicit model. A Generalized Gradient Approximation functional, PBE (Perdew-Burke-Erzerhof), and the Ahlrichs' def2-TZVP(-F) basis set were used for the DFT. D3BJ-Atom-pairwise dispersion correction to the DFT energy with Becke-Johnson damping was included to account for the Van der Waals/London dispersion forces in the interactions. All the energies were converged to the default TIGHTSCF setting of $10^{-8}$ atomic units. Frequency calculations were done to confirm that there are no negative frequencies and the optimization is indeed the ground state. For all the cases, the "restricted" approach was used.   
% % The charge on the pristine chini cluster was set to -2, and for studying the chini cluster-Zn(2+) interaction the charge was set to 0. The spin multiplicity was selected to be 1 (2S+1) to indicate the singlet state of the systems. 

% The above parameters were also used for the optimization of initial Zn-Chini cluster interactions to maintain uniformity of the energetics in the dataset provided to the BO optimization scheme. Further, the BO-suggested new Zn sites were optimized with the same parameters for the same reason. The Cartesian coordinate trajectories generated during the optimizations were used as input to the graph-powered BO optimizer in the form of a .xyz. 
% % The visualization of the trajectories was done using the AVOGADRO \cite{Avogadro}.
            
%             % The initial data set was created by placing Zn(2+) ions on the chemically distinct sites and were selected to cover all the whole cluster surface interactions. The chemically distinct sites in Pt3 were found to be - 
%             % And in Pt6 were found to be . Similarly, for Pt9 the chemicall distinct sites were found to be - 
            
 
% \subsection{ System 2: Zn oxide Nanoclusters}

% % 

% The DFT calculations for (ZnO)$_{78}$ nanoclusters are performed using the quantum chemistry and solid-state physics software package CP2K \cite{Kuhne.2020}, in version 9.1. The (ZnO)$_{78}$ nanocluster was modeled within an orthorhombic cell with dimensions $28.878 \times 26.277 \times 26.054$ \AA, which was seen to provide sufficient space to minimize interactions between periodic images from our benchmark study. Periodic boundary conditions (PBC) were applied in all three spatial directions to simulate an extended system. Geometry optimizations were performed using the BFGS algorithm with the following convergence criteria:
% \begin{itemize}
%     \item Maximum displacement: $3.0 \times 10^{-3}$ \AA
%     \item Maximum force: \SI{4.5e-4}{\hartree\per\bohr}
%     \item RMS displacement: \SI{1.5e-3}{\angstrom}
%     \item RMS force: $3.0 \times 10^{-4}$ Ha/Bohr
% \end{itemize}

% The Perdew-Burke-Ernzerhof (PBE) \cite{PBE} functional was employed to describe exchange-correlation interactions. Additionally, van der Waals (vdW) interactions were included using the DFT-D3 method with Becke-Johnson damping (DFTD3(BJ)). The DZVP-MOLOPT-SR-GTH basis sets, developed by VandeVondele and Hutter \cite{VandeVondele.2007} were used for Zn, O, and C atoms, along with the GTH-PBE pseudopotentials \cite{Hartwigsen1998, Goedecker1996} to represent the core electrons of the respective atoms.

% All structures were relaxed until the forces in the system were below \SI{4.50e-4}{\hartree\per\bohr} ($= \SI{2.31e-2}{\electronvolt\per\angstrom}$), with \si{\bohr} being the Bohr radius. For CP2K's Quickstep module, a cutoff value of \SI{900}{\rydberg} in combination with a relative cutoff value of \SI{80}{\rydberg} were found to give accurate and converged results. For the electrostatic potential, the periodic Poisson solver was utilized to handle the periodic boundary conditions in all three dimensions, ensuring the accurate computation of long-range interactions. The entire framework, including creating the input files and post-processing the results, is programmed in Python.


% All calculations were performed using the CP2K package version 9.1 \cite{Kuhne.2020}. The focus of the study was to investigate the adsorption of CO on a ((ZnO)$_{78}$)$_{78}$ nanocluster using Density Functional Theory (DFT). The computational setup and parameters were carefully chosen to ensure accurate and reliable results.
% The ((ZnO)$_{78}$)$_{78}$ nanocluster was modeled within an orthorhombic cell with dimensions 28.878 × 26.277 × 26.054 Å, which provides sufficient space to minimize interactions between periodic images. Periodic boundary conditions (PBC) were applied in all three spatial directions to simulate an extended system. 
% Geometry optimizations were performed using the BFGS algorithm with the following convergence criteria: Maximum displacement: $3.0 × 1 0 − 3 3.0×10 −3 Å Maximum force: 4.5 × 1 0 − 4 4.5×10 −4 Ha/Bohr RMS displacement: 1.5 × 1 0 − 3 1.5×10 −3 Å RMS force: 3.0 × 1 0 − 4 3.0×10 −4 Ha/Bohr$ A maximum of 400 optimization iterations were allowed. The Perdew-Burke-Ernzerhof (PBE) functional was employed to describe exchange-correlation interactions. Additionally, van der Waals (vdW) interactions were included using the DFT-D3 method with Becke-Johnson damping (DFTD3(BJ)), which is particularly important for accurately modeling adsorption phenomena. The DZVP-MOLOPT-SR-GTH basis sets were used for Zn, O, and C atoms, along with the GTH-PBE pseudopotentials to represent the core electrons . The choice of these basis sets balances computational efficiency with accuracy in describing the electronic structure of the ((ZnO)$_{78}$)$_{78}$ cluster.
% For the electrostatic potential, the periodic Poisson solver was utilized to handle the periodic boundary conditions in all three dimensions, ensuring the accurate computation of long-range interactions. A multigrid approach with 5 levels and a primary grid cutoff of 900 Ry, and a relative cutoff of 80 Ry, was adopted to ensure accurate integration of the electronic density and potential .



 



==> latexmkrc <==
# This file is part of the TUM Overleaf template.
# It is used to point the LaTeX Compiler to the class and package files
# located in the tum/ subdirectory.

$ENV{'TEXINPUTS'}='./tum//:' . $ENV{'TEXINPUTS'};
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
